GraphChain: Large Language Models for Large-scale Graph Analysis via Tool Chaining

Large Language Models (LLMs) face significant limitations when applied to large-scale graphs, struggling with context constraints and inflexible reasoning. We present GraphChain, a framework that enables LLMs to analyze complex graphs through dynamic sequences of specialized tools, mimicking human exploratory intelligence. Our approach introduces two key innovations: (1) Progressive Graph Distillation, a reinforcement learning mechanism that generates optimized tool sequences balancing task relevance with information compression, and (2) Structure-aware Test-Time Adaptation, which efficiently tailors tool selection strategies to diverse graph topologies using spectral properties and lightweight adapters without costly retraining. Experiments show GraphChain significantly outperforms prior methods, enabling scalable and adaptive LLM-driven graph analysis.

==> data/experiment_ori.tex <==
\section{Experiment}
\label{sec:experiment}
\subsection{Experimental Setting}
\textbf{Graph Dataset.} We evaluate GraphChain on five diverse graph datasets representing different real-world domains as shown in Table~\ref{tab:dataset_stats}. 
\begin{table}[h]
\centering
\caption{Statistics of graph datasets used in our experiments.}
\vspace{0.5em}
\label{tab:dataset_stats}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccclp{4.5cm}@{}}
\toprule
\textbf{Scenario} & \textbf{Dataset} & \textbf{\#Nodes} & \textbf{\#Edges} & \textbf{\#Features} & \textbf{Type} & \textbf{Description} \\
\midrule
\multirow{3}{*}{Citation Graps} & Cora & 2,708 & 10,556 & 1,433 & \multirow{3}{*}{Directed} & \multirow{3}{4.5cm}{Academic papers connected by citation relationships \citep{yang2016revisiting}} \\
 & CiteSeer & 3,327 & 9,104 & 3,703 & & \\
 & PubMed & 19,717 & 88,648 & 500 & & \\
\midrule
\multirow{2}{*}{Social Networks} & Facebook & 4,039 & 88,234 & - & Undirected & \multirow{2}{4.5cm}{Online interactions ~\citep{leskovec2012learning}} \\
 & Twitter & 81,306 & 1,768,149 & - & Directed & \\
\midrule
Chemical Molecules & QM9 & $\sim$18.0/graph & $\sim$37.3/graph & 11 & Undirected & Molecular structures with bonds between atoms \citep{wu2018moleculenet} \\
\midrule
Traffic Networks & METR-LA & 207 & 1,515 & - & Directed & Road networks with geographic constraints \citep{chen2020multi} \\
\midrule
Financial Networks & Elliptic & 203,769 & 234,355 & 165 & Directed & Transaction networks~\citep{weber2019anti} \\
\bottomrule
\end{tabular}%
}
\end{table}


\textbf{Instruction Data.}
We constructed two complementary instruction datasets: (1) an SFT dataset comprising 9986 (query, tool sequence, answer) triplets based on 45 carefully selected NetworkX functions\footnote{https://networkx.org}, and (2) an RL dataset containing 3,000 expert-annotated (query, answer) pairs (600 per graph scenario). The SFT dataset serves as the foundation for training the base model to generate appropriate tool sequences from natural language queries. For the RL dataset, we allocated 500 pairs per scenario for training and 100 for testing. Domain experts crafted exemplary instruction templates to ensure ecological validity across diverse reasoning patterns and complexity levels. Please refer to Appendix~\ref{app:data_construction} for more detail.

\textbf{Baselines.}
We conducted a comprehensive evaluation of GraphChain against state-of-the-art methods from two categories: Text-Instruction and Tool-Instruction approaches (Appendix~\ref{app:baseline}).

For Text-Instruction methods, we evaluated leading closed-source LLMs (Claude-series~\citep{TheC3}, GPT-series~\citep{DBLP:journals/corr/abs-2303-08774}) and GLM4-0520~\citep{glm2024chatglm} using two-shot prompting with Chain-of-Thought reasoning, and reproduced specialized graph reasoning methods (NLGraph~\citep{DBLP:conf/nips/WangFHTHT23}, GraphWiz~\citep{DBLP:journals/corr/abs-2402-16029}). Due to context window limitations, we restricted these experiments to small-scale graph instances, using subgraphs split from larger networks and molecular graphs.
For Tool-Instruction methods, we compared against recent tool-augmented approaches (Graph-ToolFormer~\citep{DBLP:journals/corr/abs-2304-11116}, GraphForge~\citep{wang2024graphtool}). 

To facilitate fair comparisons with existing methods—all of which require loading the entire graph into the context window—we partitioned the original graph data into subgraphs containing fewer than 100 nodes. This approach enables direct comparative analysis between our method and existing approaches under equivalent conditions.
In a separate scalability experiment (Section~\ref{subsec:scalibility}), we demonstrate that our method maintains performance comparable to small-scale graphs even when scaling to graphs with approximately 200,000 nodes, highlighting the exceptional scalability of GraphChain.

\textbf{Training Setup.}
We used two NVIDIA A800 GPUs to perform LoRA-based fine-tuning (rank $r$=16, alpha=32) on the Qwen2.5-7B-instruction model to obtain GraphChain. 
For SFT stage, we used a learning rate of $5e-5$ with $4\%$ warmup and a cosine scheduler for $5$ epochs.
For RL stage, we configured a learning rate of $1e-5$, batch size of 8, and initial KL coefficient of 0.3. Our PPO implementation followed standard practices with GAE ($\lambda$=0.95) and discount factor ($\gamma$=0.99).
During inference, we used a temperature of 0.7 and top-p value of 1.0. 
Further details on experiment settings are provided in Appendix~\ref{app:baseline}. 


\subsection{Main Results}

\begin{table}[t]
\centering
\caption{Performance comparison (accuracy \%) across five real-world graph reasoning scenarios.}
\vspace{0.5em}
\label{tab:main_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multicolumn{8}{c}{\textbf{Text-Instruction Methods}} \\
\midrule
\textbf{Model} & \textbf{Parameters} & \textbf{Financial Network} & \textbf{Chemical Molecule} & \textbf{Social Network} & \textbf{Citation Graph} & \textbf{Traffic Network} & \textbf{Average} \\
\midrule
Claude-3-Sonnet & 137B & 21.7 $\pm$ 1.8& 47.0 $\pm$ 2.2 & 21.5 $\pm$ 3.2& 17.7 $\pm$ 2.1& 16.8 $\pm$ 2.0& 24.9 $\pm$ 2.3 \\
GPT-3.5-turbo & $\sim$175B & 36.6 $\pm$ 2.1& 23.0 $\pm$ 3.7& 18.2 $\pm$ 3.6& 12.2 $\pm$ 0.8& 19.4 $\pm$ 1.9& 21.9 $\pm$ 2.4\\
Claude-3-Haiku & 43B & 12.2 $\pm$ 3.0& 52.9 $\pm$ 3.2& 50.3 $\pm$ 3.4& 19.8 $\pm$ 2.0& 13.9 $\pm$ 2.4& 29.8 $\pm$ 2.8\\
Claude-3-Opus & 175B & 23.6 $\pm$ 2.1& 42.4 $\pm$ 1.4& 51.9 $\pm$ 1.3& 36.7$\pm$ 3.1& 43.4 $\pm$ 3.3& 39.6 $\pm$ 2.2\\
GraphWiz & 13B & 41.1 $\pm$ 3.9& 52.4 $\pm$ 2.6& 61.5 $\pm$ 3.5& 68.0 $\pm$ 2.1& 38.4 $\pm$ 1.9& 52.3 $\pm$ 2.9\\
NLGraph & - & 52.1 $\pm$ 3.4& 58.4 $\pm$ 2.5& 65.2 $\pm$ 2.3& 59.4 $\pm$ 0.5& 39.8 $\pm$ 1.8& 55.0 $\pm$ 2.1\\
GPT-4o & $\sim$1.8T & 57.5 $\pm$ 1.9& 62.7 $\pm$ 3.6& 65.2 $\pm$ 3.9& \underline{71.5 $\pm$ 3.4}& 43.4 $\pm$ 1.6 & 59.4 $\pm$ 2.6 \\
\midrule
\multicolumn{8}{c}{\textbf{Tool-Instruction Methods}} \\
\midrule
Graph-ToolFormer & 6B & 47.5 $\pm$ 1.9& 68.1 $\pm$ 4.8& 74.7 $\pm$ 4.2& 61.4 $\pm$ 3.4& 65.8 $\pm$ 4.5& 62.4 $\pm$ 3.5\\
GraphForge & 8B & \underline{63.5 $\pm$ 3.5}& \underline{70.9 $\pm$ 5.4}& \underline{80.4 $\pm$ 4.2}& 63.4 $\pm$ 4.4& \underline{73.5 $\pm$ 3.1}& \underline{70.2 $\pm$ 3.8}\\
\midrule
GraphChain & 7B & \textbf{81.5 $\pm$ 2.2} & \textbf{81.1 $\pm$ 0.7} & \textbf{89.6 $\pm$ 2.0} & \textbf{83.6 $\pm$ 2.6} & \textbf{84.1 $\pm$ 0.3} & \textbf{84.7 $\pm$ 1.8} \\
\midrule
\textit{Relative improvement (\%)} & - & \textit{+28.3\%} & \textit{+14.4\%} & \textit{+11.4\%} & \textit{+16.9\%} & \textit{+14.4\%} & \textit{+20.7\%} \\
\bottomrule
\multicolumn{8}{r}{\scriptsize{$^\dagger$ \textbf{Boldface} denotes the highest score, and \underline{underline} indicates the best result among baselines.}}
\end{tabular}%
}
\end{table}

Table~\ref{tab:main_results} presents a comprehensive performance comparison of GraphChain against state-of-the-art baselines across five diverse graph reasoning scenarios. 
Statistical analysis using two-sample t-tests confirms that these improvements are statistically significant ($p < 0.05$).

Our empirical evaluation reveals several key insights:

\begin{itemize}[leftmargin=*]
    \item GraphChain substantially outperforms all baselines across both categories, achieving 84.7\% average accuracy compared to 70.2\% for the best baseline (GraphForge), representing a 20.7\% relative improvement.
    \item Among the text-instruction baselines, GPT-4o with approximately 1.8T parameters demonstrates superior performance (59.4\% average accuracy), corroborating the applicability of scaling laws to graph reasoning tasks. 
    \item When confronted with tool-instruction methods, specialized graph reasoning approaches like GraphForge (70.2\% average accuracy) significantly outperform even the largest general-purpose LLMs.
    \item Notably, GraphChain achieves these results with only 7B parameters, compared to GraphForge's 8B and GPT-4o's ~1.8T. This parameter efficiency, combined with superior performance.
\end{itemize}



\subsection{Ablation Study}
To rigorously evaluate the contribution of each component in GraphChain, we conducted a systematic ablation study by introducing two principal variants of the model: (1) \textbf{w/o graph distillation}, where the reward associated with information distillation during training is set to zero, effectively disabling the progressive graph distillation mechanism; and (2) \textbf{w/o test-time adaptation}, where the Structure-aware Test-Time Adaptation (STTA) component is entirely removed during inference.

\begin{figure}[t]
\centering
\begin{minipage}{0.4\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/ablation_bywangxin.pdf}
   \caption{Impact of removing graph distillation or test-time adaptation components from GraphChain.}
   \label{fig:ablation}
\end{minipage}
\hfill
\begin{minipage}{0.5\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/complexity_bywangxin.pdf}
   \caption{Comparison with varying Graph Sizes and Query Complexity.}
   \label{fig:complexity}
\end{minipage}
\end{figure}

Figure~\ref{fig:ablation} reveals several key insights about GraphChain's components:

\begin{itemize}[leftmargin=*]
   \item GraphChain consistently outperforms GraphForge across all graph scenarios, demonstrating the superiority of our approach over existing graph tool-calling methods.
   
   \item Removing either graph distillation or test-time adaptation leads to performance degradation, confirming that both components play critical roles in enabling effective tool-chaining and structural understanding of graphs.
   
   \item The performance drop is substantially more severe when graph distillation is removed compared to when test-time adaptation is disabled. This observation highlights that efficient tool sequence generation through progressive distillation is particularly crucial for graph analysis tasks. Even without test-time adaptation, the model can still leverage its general knowledge to explore graph information through tool-chaining, albeit less effectively.
   
   \item Notably, GraphChain without test-time adaptation still outperforms GraphForge in most scenarios, indicating that our multi-step tool-chaining approach with graph distillation is inherently more effective than single-step tool invocation patterns when addressing complex graph analysis.
\end{itemize}

\subsection{Scalability Analysis}
\label{subsec:scalibility}
To systematically evaluate GraphChain's capabilities across varying levels of complexity, we stratified our evaluation dataset into distinct groups based on graph size (measured by node count) and reasoning complexity (measured by tool sequence length), enabling precise assessment of how performance scales with these critical dimensions. Figure~\ref{fig:complexity} reveals several important findings about GraphChain's scalability advantages:
\begin{itemize}[leftmargin=*]
   \item As graph size increases, both baseline methods exhibit significant performance degradation, with GPT-4o declining more dramatically. This demonstrates the limitations of text-instruction methods when confronted with larger graph structures. 
   
   \item Notably, GraphChain sustains its performance advantage consistently across the entire range of graph sizes tested, including graphs with up to 200,000 nodes. This exceptional scalability stems from our approach of representing memory states through concise natural language summaries rather than direct graph descriptions, enabling effective reasoning over graph structures that far exceed context window limitations.
   
   \item While all methods perform reasonably well on simple queries (requiring 1-2 tool calls), performance disparities become increasingly pronounced as query complexity increases. Both GPT-4o and GraphForge show steep performance declines for queries requiring 4-5 tool calls, while GraphChain maintains substantially higher accuracy. This demonstrates GraphChain's superior capability for multi-step reasoning through its progressive graph distillation mechanism.
\end{itemize}


\subsection{Transfer Learning Evaluation}

To assess GraphChain's transfer capabilities, we conducted cross-domain experiments by fine-tuning the model exclusively on Financial Network instructions and evaluating on three unseen domains: Social Network, Citation Graph, and Traffic Network. We compared performance with and without the Structure-aware Test-Time Adaptation (STTA) module to isolate its contribution to domain adaptation.

\begin{table}[h]
\centering
\small
\caption{Results (accuracy \%) when training on Financial Network and testing on other domains.}
\label{tab:transfer}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Social Network} & \textbf{Citation Graph} & \textbf{Traffic Network} \\
\midrule
GraphChain (in-domain) & 89.6 & 83.6 & 84.1 \\
GraphChain w/ STTA & 86.8 (-3.1\%) & 79.2 (-4.3\%) & 80.3 (-4.5\%) \\
GraphChain w/o STTA & 84.5 (-5.7\%) & 75.1 (-10.2\%) & 77.4 (-8.0\%) \\
\bottomrule
\end{tabular}
\end{table}

Results in Table~\ref{tab:transfer} demonstrate GraphChain's strong transfer learning capabilities, with cross-domain performance closely approaching in-domain results. The Structure-aware Test-Time Adaptation mechanism substantially improves transfer performance, reducing accuracy drops by 2.6\%, 5.9\%, and 3.5\% across the three target domains compared to the variant without STTA. This confirms STTA's effectiveness in dynamically adapting to diverse graph structures, enabling robust generalization to previously unseen graph domains without domain-specific retraining.
\begin{figure}[h]
    \centering
    \includegraphics[page=1,width=0.9\textwidth]{figures/casestudy.pdf}
    \caption{A typical case of GraphChain.}
\end{figure}



\subsection{Tool Chain Analysis}

To understand how GraphChain adapts its exploration strategy across different graph domains, we categorized our tools into six functional clusters (Graph Statistics, Subgraph Extraction, Path Planning, Centrality Measures, Community Detection, and Connectivity) and analyzed their usage patterns across the four graph scenarios.

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/pie_bywangxin.pdf}
\caption{Distribution of tool types utilized by GraphChain across different graph domains.}
\label{fig:tool_distribution}
\end{figure}

Figure~\ref{fig:tool_distribution} reveals distinct exploration patterns adapted to each domain's characteristics. Path Planning tools dominate in Traffic Network (33.8\%) and Financial Network (26.7\%) scenarios, reflecting the importance of traversal analysis in these domains. Social Network analysis relies heavily on Centrality Measures (28.8\%) and Community Detection (20.4\%), aligning with the importance of influence and clustering in social structures. Citation Graph processing shows a more balanced distribution with significant usage of Connectivity tools (18.9\%), highlighting the importance of reachability in citation networks. 

These domain-specific variations demonstrate GraphChain's ability to adaptively construct appropriate tool sequences based on graph topology, supporting our assertion that the progressive graph distillation mechanism effectively captures and exploits domain-specific structural patterns through informed tool selection.


\subsection{Case Study}

In this subsection, we present a case study of a transmission network scenario, which is characterized by a multi-directional graph with weighted edges. This graph is taken from a part of the Elliptic Dataset and consists of 11,896 nodes and 31,054 edges. Obviously, this exceeds the context processing capabilities of current mainstream LLMs. Additionally, due to the complexity of the problem that cannot be solved through a single tool invocation, it is difficult for GraphToolFormer and GraphForge to obtain the true answer.

In contrast, our proposed GraphChain framework demonstrates a robust capability to systematically handle such tasks. GraphChain provides a clear and accurate solution through a series of tool invocations. The Progressive Graph Distillation mechanism enables GraphChain to iteratively reduce the information complexity of the graph and focus on the most salient features of the task at hand. 

Due to the limitations of the context window in large language models, we store the processing results of intermediate steps in memory rather than directly inputting them into the large model. At this point, the large language model outputs a detailed description of the current step's processing results and its usage methods to facilitate further analysis and processing. Only when the number of tokens in the intermediate step's results is less than the maximum context window limit of the large model will the intermediate results be directly input into the large language model. This can maximizes the advantages of the large language model and minimizes its disadvantages.

This case study underscores GraphChain's ability to systematically explore and analyze large-scale graphs, affirming its feasibility for tackling complex graph-based problems. The model's success in accurately addressing real-world graph tasks highlights its substantial practical value, positioning GraphChain as a transformative approach for LLM-augmented graph processing.







==> data/methodology_ori.tex <==
\section{Methodology}
\label{sec:methodology}



\begin{figure}[!t]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/framework.pdf}
  \caption{\small \textbf{(1) Training Phase:} Implements progressive graph distillation where the RL agent learns to select tool sequences progressively reducing the memory state's ($\mathbf{m}$) Graph Description Length (GDL) and maximizing task relevance. \textbf{(2) Structure-aware Test-Time Adaptation:} Employs a lightweight adapter ($\mathcal{A}_{\psi}$) tuned via minimizing chain length and KL divergence. The adapter generates a structure-specific soft prompt $\mathbf{P}_G$ based on the graph's SVD-derived fingerprint $\mathbf{z}_G$.}
  \label{fig:framework}
\end{figure}



GraphChain tackles the inherent difficulties of applying Large Language Models (LLMs) to large-scale graph analysis by formulating the problem as a sequential decision-making task solvable via reinforcement learning (RL). 
The effectiveness of GraphChain stems from two core technical innovations designed to overcome the primary challenges identified in Section~\ref{sec:intro}: (1) \textbf{Progressive Graph Distillation}, an RL training mechanism promoting informative yet compact state representations, and (2) \textbf{Structure-aware Test-Time Adaptation}, enabling the agent to dynamically adjust its strategy to diverse graph topologies using soft prompts. A conceptual overview is provided in Figure~\ref{fig:framework}.


\subsection{Progressive Graph Distillation}
\label{sec:distillation_rl}

Generating effective tool sequences for complex graph queries involves navigating an exponentially large action space, a challenge compounded by potentially sparse rewards derived only from final task completion. To furnish denser learning signals and emulate efficient analytical workflows---akin to human strategies that often proceed from coarse-grained overviews to fine-grained details---we introduce \textbf{Progressive Graph Distillation}.

The core principle is to incentivize the RL agent to concurrently pursue the query objective and actively manage the complexity of its intermediate memory state $\mathbf{m}$. We train the agent to prioritize tool sequences that systematically \textit{reduce the data volume} of $\mathbf{m}$ while retaining task-critical information pertinent to the query $\mathcal{Q}$. This transforms the exploration process into a guided search characterized by iterative refinement. The aim is to progressively shrink the memory state $\mathbf{m}$ step-by-step, eventually yielding a final state $\mathbf{m}_N$ that is sufficiently compact for direct processing within the LLM's context window, facilitating final answer generation.


\subsubsection{Quantifying Memory State Volume and Relevance} % Changed Complexity to Volume
\label{sec:volume_relevance} % Updated label to match title change

Implementing progressive distillation requires quantifying two key aspects of the memory state $\mathbf{m}_t$ at each step $t$: its \textbf{data volume} (size) and its \textbf{relevance} to the query $\mathcal{Q}$.

\paragraph{Graph Description Length ($\mathrm{GDL}(\mathbf{m}_t)$):} We require a principled metric reflecting the data volume or information cost associated with storing the intermediate graph state in memory $\mathbf{m}_t$. Drawing inspiration from the Minimum Description Length (MDL) principle~\cite{barron1998minimum}, which favors models enabling the most compact data representation, we introduce the concept of Graph Description Length (GDL). This metric serves as a proxy for the data size required to represent the current graph state. Assuming the primary components of the memory state $\mathbf{m}_t$ are a subgraph $G'_t = (\mathcal{V}'_t, \mathcal{E}'_t)$ with $n'_t = |\mathcal{V}'_t|$ nodes and $m'_t = |\mathcal{E}'_t|$ edges, along with associated node features $\mathbf{X}'_t \in \mathbb{R}^{n'_t \times d_f}$, we define the GDL as the sum of terms approximating the space needed for structure and features:
\begin{equation}
\mathrm{GDL}(\mathbf{m}_t) = L(\text{structure}) + L(\text{features}) \approx \alpha_s m'_t + \alpha_f n'_t d_f
\label{eq:memory_gdl}
\end{equation}
The coefficients $\alpha_s, \alpha_f \ge 0$ allow for weighting the relative contribution of structural versus feature information to the overall data volume. 
% The objective within our progressive distillation framework is to encourage trajectories where $\mathrm{GDL}(\mathbf{m}_t)$ is minimized or reduced over time, promoting concise yet informative intermediate states.

\paragraph{Task Relevance ($\mathrm{Rel}(\mathbf{m}_t, \mathcal{Q})$):} Assessing the utility of the current memory state $\mathbf{m}_t$ for answering the query $\mathcal{Q}$ is crucial. Directly computing the mutual information $I(\mathbf{m}_t; \mathcal{A}_{\mathcal{Q}})$ (where $\mathcal{A}_{\mathcal{Q}}$ is the true answer) is generally intractable. Therefore, we employ a practical proxy using an auxiliary LLM scorer. Since $\mathbf{m}_t$ itself, which may contain large subgraphs or embeddings, can exceed the LLM's context limits, we leverage the concise natural language description $d_t$ produced by the executed tool $T$ (as defined in Eq.~\ref{eq:tool_function}). This description $d_t$ acts as a compressed, LLM-interpretable summary of the information gain or state change resulting from the tool's operation. We estimate the task relevance at step $t$, denoted $\mathrm{Rel}(\mathbf{m}_t, \mathcal{Q})$, by prompting the LLM scorer with the original query $\mathcal{Q}$, the history of preceding descriptions $H_t = \{d_0, \dots, d_{t-1}\}$, and the most recent description $d_t$:
\begin{equation} % Changed symbol from \hat{R}_t to Rel_t
\mathrm{Rel}(\mathbf{m}_t, \mathcal{Q}) \approx \text{LLMScore}(\text{prompt}(\mathcal{Q}, H_t, d_t)) \in [0, 1]
\label{eq:task_relevance}
\end{equation}
% This relevance estimate $\mathrm{Rel}(\mathbf{m}_t, \mathcal{Q})$ guides the agent towards actions that yield summaries deemed valuable by the LLM scorer in the context of the ongoing analysis for query $\mathcal{Q}$. % Updated final sentence with new symbol

\subsubsection{Distillation-based Reward Shaping}
\label{sec:reward_design}

We incorporate the principles of progressive distillation directly into the RL reward function $R_t = R(s_t, a_t, s_{t+1})$. The reward structure is designed to provide denser feedback during the exploration process while also assessing final task completion. We define $R_t$ conditionally based on whether the process is ongoing ($t < N$) or has terminated ($t = N$):

\begin{equation}
R_t =
\begin{cases}
w_1 \cdot \hat{r}^{\mathrm{Succ}}_t + w_2 \cdot \hat{r}^{\Delta \mathrm{GDL}}_t + w_3 \cdot \hat{r}^{\Delta \mathrm{Rel}}_t & \text{if } t < N \\
w_{\text{solve}} \cdot \mathrm{EvaluateTaskSuccess}(\mathcal{Q}, s_{N+1}) & \text{if } t = N
\end{cases}
\label{eq:unified_reward_distill} % Changed label for new unified equation
\end{equation}
where $N$ is the final step index upon termination, and the components for the intermediate reward ($t < N$) are defined as follows:

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
    \item $\hat{r}^{\mathrm{Succ}}_t = \mathbb{I}(\textit{ExecutionSuccess}(a_t, s_{t+1}))$ is a binary reward for valid tool execution.
    % , where $\mathbb{I}(\cdot)$ is the indicator function.

    \item $\hat{r}^{\Delta \mathrm{GDL}}_t$ rewards the reduction in the relative Graph Description Length (GDL) of the memory state, normalized to a bounded range using the $\tanh$ function. This scaling ensures the GDL reduction reward component is comparable in magnitude to other components:
    \begin{equation}
      \hat{r}^{\Delta \mathrm{GDL}}_t = \tanh\left(\beta \frac{\mathrm{GDL}(\mathbf{m}_{t-1}) - \mathrm{GDL}(\mathbf{m}_t)}{\mathrm{GDL}(\mathbf{m}_{t-1}) + \epsilon}\right)
      \label{eq:gdl_reward_normalized}
    \end{equation}
    Here, $\mathrm{GDL}(\mathbf{m})$ is defined in Eq.~\ref{eq:memory_gdl}, $\beta > 0$ is a scaling hyperparameter controlling the sensitivity of the reward to relative GDL changes, and $\epsilon > 0$ is a small constant for numerical stability. The output is bounded within $(-1, 1)$, rewarding reduction (positive value) and penalizing increase (negative value) in relative GDL.

    \item $\hat{r}^{\Delta \mathrm{Rel}}_t = \text{Rel}_t - \text{Rel}_{t-1}$ rewards the increase in the estimated task relevance, using the relevance proxy $\text{Rel}_t$ defined in Eq.~\ref{eq:task_relevance}. This incentivizes actions that yield more informative states regarding the query $\mathcal{Q}$. This value is naturally bounded within $[-1, 1]$ as $\text{Rel}_t \in [0, 1]$.
\end{itemize}

The non-negative weights $w_1, w_2, w_3$ balance the importance of successful execution, memory volume reduction (via GDL), and relevance gain during the intermediate steps. The weight $w_{\text{solve}}$ scales the final reward obtained upon termination ($t=N$), which assesses the overall success in addressing the query $\mathcal{Q}$ based on the final state $s_{N+1}$. 
% This structured, conditional reward signal guides the agent towards generating tool sequences that are not only effective in solving the task but also efficient in managing intermediate data complexity, aligning with the progressive distillation objective.

\subsubsection{Information Bottleneck Perspective}
\label{sec:info_bottleneck}

The design of our progressive distillation mechanism, particularly the reward structure defined in Eq.~(\ref{eq:unified_reward_distill}), can be intuitively understood through the lens of the Information Bottleneck (IB) principle \citep{tishby2010information}. The IB principle advocates for learning representations that are maximally informative about a target variable while being maximally compressive with respect to the input. Our reward function operationalizes this trade-off by incentivizing high task relevance (estimated via $\mathrm{Rel}_t$, Eq.~\ref{eq:task_relevance}) while simultaneously rewarding reductions in state volume (measured by $\mathrm{GDL}(\mathbf{m}_t)$, Eq.~\ref{eq:memory_gdl}).

This process implicitly encourages the agent to learn a policy that generates intermediate memory states $\mathbf{m}_t$ which act as information bottlenecks. The following proposition formalizes the intuition that optimizing our reward structure preferentially discards task-irrelevant information.

\begin{proposition}
\label{prop:ib_compression}
Let the input be $X=(G, \mathcal{Q})$, containing task-relevant information $Y=\mathcal{A}_{\mathcal{Q}}$ (the answer) and task-irrelevant information $IR$, with the Markov structure $(Y, IR) \rightarrow X \rightarrow \mathbf{m}_t$. Assuming the relevance proxy $\mathrm{Rel}_t$ positively correlates with the mutual information $I(\mathbf{m}_t; Y)$ and the GDL serves as a measure of complexity encouraging smaller $I(X; \mathbf{m}_t)$, optimizing the policy $\pi_\phi$ with the reward function $R_t$ (Eq.~\ref{eq:unified_reward_distill}) guides the generation of memory states $\mathbf{m}_t$ that tend to minimize the irrelevant information $I(N; \mathbf{m}_t | Y)$ while preserving the relevant information $I(\mathbf{m}_t; Y)$.
\end{proposition}

Detailed proof is provided in Appendix~\ref{app:proof_ib_prop}. Proposition~\ref{prop:ib_compression} provides theoretical backing for our distillation approach. By rewarding both relevance gain and volume reduction, the RL process steers the agent towards behaviours that effectively filter the graph data. Our framework learns to intentionally reduce the representational footprint of task-irrelevant graph components (e.g., distracting structures or features) while preserving information critical to answering the query $\mathcal{Q}$. This selective compression is key to generating concise intermediate states $\mathbf{m}_t$, mitigating context exhaustion and enabling effective analysis of large graphs.


\subsubsection{Policy Optimization}
\label{sec:policy_opt}

To optimize the LLM agent's policy $\pi_\phi$, parameterized by $\phi$, our framework can accommodate various policy gradient algorithms. In practice, we implement Proximal Policy Optimization (PPO)~\citep{schulman2017proximal}, an actor-critic method recognized for its balance of sample efficiency and training stability. PPO requires estimating the advantage function, for which we utilize Generalized Advantage Estimation (GAE)~\citep{schulman2015high} for improved stability:
\begin{equation}
\hat{A}_t^{\text{GAE}}(\phi, \omega) = \sum_{l=0}^{N-t} (\gamma\lambda)^l \delta_{t+l}, \quad \text{where} \quad \delta_t = R_{t+1} + \gamma V_\omega(s_{t+1}) - V_\omega(s_t)
\label{eq:gae_distill_revised}
\end{equation}
Here, $\lambda \in [0, 1]$ is the GAE trace decay parameter, $V_\omega$ is the learned value function parameterized by $\omega$, $\gamma$ is the discount factor, and $R_{t+1}$ represents the distillation-aware reward (Eq.~\ref{eq:unified_reward_distill}).

Following the PPO-clip approach~\citep{schulman2017proximal}, we optimize the policy by maximizing a clipped surrogate objective. Adapting the structure presented in related works for complex action sequences, the policy objective $\mathcal{L}^{\text{CLIP}}$ can be expressed based on trajectories $\tau$ sampled from the policy $\pi_\phi$:
\begin{equation}
\mathcal{L}^{\text{CLIP}}(\phi) = \hat{\mathbb{E}}_{\tau \sim \pi_\phi} \left[ \sum_{t=0}^{N} \min \left( \frac{\pi_\phi(a_t|s_t)}{\pi_{\phi_{\text{old}}}(a_t|s_t)} \hat{A}_t^{\text{GAE}}, \, \text{clip}\left(\frac{\pi_\phi(a_t|s_t)}{\pi_{\phi_{\text{old}}}(a_t|s_t)}, 1 - \epsilon, 1 + \epsilon \right) \hat{A}_t^{\text{GAE}} \right) \right]
\label{eq:ppo_clip_obj_revised} % New label for the clip objective only
\end{equation}
where $\pi_{\phi_{\text{old}}}$ is the old policy used for generating the trajectories in the batch, $\hat{A}_t^{\text{GAE}}$ is the estimated advantage from Eq.~\ref{eq:gae_distill_revised}, and $\epsilon$ is the clipping hyperparameter. 

% The full PPO objective typically combines this policy loss with a value function loss (e.g., $\mathcal{L}^{\text{VF}}_t(\omega) = (V_\omega(s_t) - V_t^{\text{targ}})^2$) and an entropy bonus $\mathcal{S}[\pi_\phi](s_t)$ to encourage exploration, weighted by coefficients $c_1$ and $c_2$ respectively. Optimizing this objective guides the policy $\pi_\phi$ towards generating tool sequences that maximize the expected distillation-aware return, balancing task completion with memory state compression and task relevance maximization.



\subsection{Structure-aware Test-Time Adaptation}
\label{sec:stta_spt_revised} % Kept original label

Graph-structured data intrinsically exhibits significant distributional shifts across domains and applications~\citep{zhao2024graphany, garg2020generalization}. A policy $\pi_\phi$ optimized on a specific set of training graphs may thus falter when encountering novel structures at test time. To circumvent the prohibitive cost of retraining for each new graph, we propose \textbf{Structure-aware Test-Time Adaptation (STTA)}, a novel mechanism that efficiently tailors the agent's behavior by dynamically generating graph-specific soft prompts via a lightweight, adaptable network. Critically, STTA leverages self-supervised signals derived by optimizing for efficient planning—implicitly constraining tool chain length—to enhance the model's step-by-step execution confidence on the specific structure of the test graph.



\subsubsection{Graph Structural Fingerprinting}
\label{sec:fingerprint_svd_revised}

To imbue the LLM with global structural awareness for large-scale graphs that exceed context limits, we derive a concise graph fingerprint. We compute the normalized graph Laplacian $\mathbf{L} = \mathbf{I} - \mathbf{D}^{-1/2}\mathbf{A}\mathbf{D}^{-1/2}$ and consider its Singular Value Decomposition (SVD), $\mathbf{L} = \mathbf{U} \mathbf{\Sigma} \mathbf{V}^T$. The smallest singular values $\sigma_i$ (diagonal entries of $\mathbf{\Sigma}$, sorted $0 = \sigma_0 \le \sigma_1 \le \dots$) are known to capture dominant, low-frequency components reflecting macroscopic graph properties like connectivity and community structure~\citep{ramasamy2015compressive}. We define the \textbf{structural fingerprint} using these key values:
\begin{equation}
\mathbf{z}_G = (\sigma_0, \sigma_1, \ldots, \sigma_M) \in \mathbb{R}^{M+1}
\label{eq:fingerprint_definition_svd}
\end{equation}
Crucially, while full SVD is intractable for very large graphs, these $M+1$ smallest singular values (where $M \ll N$ is a hyperparameter) can be computed efficiently using iterative SVD algorithms (e.g., Lanczos bidiagonalization). This process effectively distills the essential global topology into a compact vector $\mathbf{z}_G$. This fingerprint $\mathbf{z}_G$ serves as the conditioning input for the adaptation network.

\subsubsection{Structure-Conditioned Prompt Generation} % Kept Adapter Network in title for clarity, but used symbol in text
\label{sec:spt_adapter}

Instead of relying on a discrete library, STTA employs a continuous adaptation mechanism through a dedicated adapter network $\mathcal{A}_{\psi}$. This network, parameterized by $\psi$, learns a mapping from the graph's structural fingerprint $\mathbf{z}_G$ (Eq.~\ref{eq:fingerprint_definition_svd}) to a corresponding soft prompt $\mathbf{P}_G \in \mathbb{R}^{L_p \times d_{emb}}$, where $L_p$ is the prompt length and $d_{emb}$ is the LLM's input embedding dimension:
\begin{equation}
\mathbf{P}_G = \mathcal{A}_{\psi}(\mathbf{z}_G)
\label{eq:adapter_generation}
\end{equation}
This generated soft prompt $\mathbf{P}_G$ is then prepended to the standard embedding $E(s_t)$ of the agent's state $s_t$, modifying the input to the frozen LLM policy network $\pi_\phi$:
\begin{equation}
\text{LLMInput}(s_t, G) = [\mathbf{P}_G ; E(s_t)] = [\mathcal{A}_{\psi}(\mathbf{z}_G) ; E(s_t)]
\label{eq:spt_input_adapter}
\end{equation}
The agent's action $a_t$ is subsequently sampled from the policy conditioned on this augmented input: $a_t \sim \pi_\phi(\cdot | [\mathcal{A}_{\psi}(\mathbf{z}_G) ; E(s_t)])$. Crucially, during test-time adaptation, the base LLM policy parameters $\phi$ remain frozen. Only the significantly smaller set of adapter parameters $\psi$ are tuned, enabling efficient adaptation.

\subsubsection{Self-Supervised Adaption}
\label{sec:tta_self_supervised}

Given the absence of ground-truth rewards for the user query $\mathcal{Q}$ on an unseen test graph $G_{\text{test}}$, STTA employs a self-supervised strategy using auxiliary queries. We leverage a general-purpose LLM ($\text{LLM}_{\text{gen}}$) to generate diverse auxiliary graph analysis queries $\{\mathcal{Q}_{\text{aux}, i}\}_{i=1}^{M}$ relevant to $G_{\text{test}}$'s structure. These queries serve as unlabeled probes to guide the adaptation.

For each $\mathcal{Q}_{\text{aux}, i}$, we perform rollouts using the frozen base policy $\pi_\phi$ conditioned on the graph-specific prompt $\mathbf{P}_{G_{\text{test}}} = \mathcal{A}_{\psi}(\mathbf{z}_{G_{\text{test}}})$, yielding trajectories $\tau_i = (s_0, a_0, \dots, s_{N_{\tau_i}})$. The adaptation of the adapter parameters $\psi$ is driven by a self-supervised objective function $L_{\text{STTA}}(\psi)$ which balances planning efficiency and policy regularization, without requiring success labels for the auxiliary tasks:

\begin{equation}
L_{\text{STTA}}(\psi) = \mathbb{E}_{\mathcal{Q}_{\text{aux}, i}, \tau_i \sim \pi_{\psi}(\cdot|s; G_{\text{test}})} \left[ w_L N_{\tau_i} + w_{KL} \sum_{t=0}^{N_{\tau_i}-1} D_{KL}(\pi_{\psi}(\cdot | s_t; G_{\text{test}}) || \pi_{\text{orig}}(\cdot | s_t)) \right]
\label{eq:stta_kl_objective} % Updated label
\end{equation}

The components of this objective are:
\begin{itemize}[leftmargin=*]
    \item \textbf{Chain Length ($N_{\tau_i}$):} The number of tool calls in the trajectory. Minimizing this term (weighted by $w_L > 0$) encourages the adapter $\mathcal{A}_{\psi}$ to generate prompts that lead to efficient planning by the policy $\pi_\phi$ on $G_{\text{test}}$.
    \item \textbf{KL Divergence Regularization:} This term (weighted by $w_{KL} > 0$) penalizes the deviation of the adapted policy's action distribution $\pi_{\psi}(\cdot | s_t; G_{\text{test}}) \approx \pi_\phi(\cdot | [\mathcal{A}_\psi(\mathbf{z}_{G_{\text{test}}}); E(s_t)])$ from the original frozen policy's distribution $\pi_{\text{orig}}(\cdot | s_t) \approx \pi_\phi(\cdot | E(s_t))$. It acts as a regularizer, ensuring the adapter induces helpful but not overly drastic changes to the base policy's behavior.
\end{itemize}

Since the chain length $N_{\tau_i}$ is non-differentiable and the objective depends on trajectory rollouts, we minimize $L_{\text{STTA}}(\psi)$ with respect to the adapter parameters $\psi$ using a policy gradient approach. Specifically, we employ the REINFORCE algorithm~\citep{williams1992simple}, consistent with optimizing based on trajectory-level feedback. Applying REINFORCE allows tuning $\mathcal{A}_{\psi}$ to generate prompts that enhance efficiency (low $N_{\tau_i}$) while maintaining fidelity to the original learned behaviors (low KL divergence), effectively adapting the frozen policy $\pi_\phi$ to the specific structure of $G_{\text{test}}$.
